3D Keypoint Estimation Using Implicit Representation Learning

In this paper, we tackle the challenging problem of 3D keypoint estimation of general objects using a novel implicit representation. Previous works have demonstrated promising results for keypoint prediction through direct coordinate regression or heatmap-based inference. However, these methods are commonly studied for specific subjects, such as human bodies and faces, which possess fixed keypoint structures. They also suffer in several practical scenarios where explicit or complete geometry is not given, including images and partial point clouds. Inspired by the recent success of advanced implicit representation in reconstruction tasks, we explore the idea of using an implicit field to represent keypoints. Specifically, our key idea is employing spheres to represent 3D keypoints, thereby enabling the learnability of the corresponding signed distance field. Explicit keypoints can be extracted subsequently by our algorithm based on the Hough transform. Quantitative and qualitative evaluations also show the superiority of our representation in terms of prediction accuracy.

==> figures/more_quali_results.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/comp_new1.png}
    \caption{The visual comparison of keypoint estimation for three types of representations (`Coords' means coordinate regression, and `Heatmap' means heatmap inference). Here, the word full or partial represents the input point cloud full (complete) or partial. Our method is based on SDF representation.}
    \label{fig:comp}
\end{figure*}

==> tables/keypoint_detection.tex <==
\begin{table*}[t]%[!t]
    \centering
    \caption{The mIoU results (in percentage) for compared keypoint detection methods with a distance threshold of 0.01. Our method utilizes the same encoder as PointNet \cite{qi2017pointnet} while adopts different keypoint representations. DGCNN \cite{wang2019dynamic} and Harris3D \cite{sipiran2011harris} are the best classification method and the best traditional method in KeypointNet \cite{you2020keypointnet}.}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
    \hline
    Method& Airplane & Bath & Chair & Car & Guitar & Knife & Laptop & Motor & Table & Vessel \\
    \hline
    Ours &\underline{19.4} & \underline{12.2} & \underline{12.5} & \underline{18.2} & \underline{17.9} & \underline{16.9} & \underline{28.0} & \underline{14.3} & \underline{25.4} & \underline{5.9} \\
    PointNet &10.4 & 0.8 & 7.7 & 7.3 & 0.1 & 0.0 & 23.6 & 0.1 & 20.9 & 7.1 \\
    DGCNN &\textbf{39.2} & \textbf{25.5} & \textbf{24.9} & \textbf{27.0} & \textbf{31.9} & \textbf{31.5} & \textbf{44.8} & \textbf{30.3} & \textbf{41.0} & \textbf{24.4} \\
    Harris3D &1.6 & 0.3 & 0.7 & 0.9 & 1.2 & 1.9 & 0.3 & 0.7 & 0.4 & 1.2 \\
    \hline     
    \end{tabular}
    
    \label{tab:mIOU}
    \vspace{-5mm}
\end{table*}

==> tables/kp_corres_comp.tex <==
\begin{table*}[ht]%[!t]
    \centering
    \caption{Comparison results for PointNet~\cite{qi2017pointnet} and RSNet~\cite{huang2018recurrent} with full point cloud inputs. Our method utilizes the same encoder as PointNet while adopts different keypoint representations. RSNet is the best of keypoint correspondence benchmark in KeypointNet~\cite{you2020keypointnet}.}
\begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c}
    \hline
    Method & Metric & Airplane & Bath & Chair & Car & Guitar & Knife & Laptop & Motor & Table & Vessel \\
    \hline
    % \multirow{2}{4em}{Ours} &BHD &0.124 & 0.235 & 0.148 & 0.121 & 0.097 & 0.147 & 0.097 & 0.194 & 0.117 & 0.260 \\
    % &CD &0.015 & 0.031 & 0.018 & 0.009 & 0.007 & 0.025 & 0.015 & 0.017 & 0.026 & 0.053 \\
    % \hline
    \multirow{2}{4em}{Ours} &BHD &\textbf{0.124} &\textbf{0.235} &\textbf{0.148} &\textbf{0.121} & 0.097 & 0.147 &\textbf{0.097} &\textbf{0.194} & 0.117 &\textbf{0.260} \\
    &CD &\textbf{0.015} &\textbf{0.031} &\textbf{0.018} &\textbf{0.009} &\textbf{0.007} &0.025 &\textbf{0.015} &\textbf{0.017} & 0.026 &\textbf{0.053} \\
    \hline
    \multirow{2}{4em}{PointNet} &BHD & 0.213 & 0.288 & 0.333 & 0.339 & \textbf{0.096} & 0.156 & 0.203 & 0.328 & \textbf{0.101} & 0.355 \\
    &CD & 0.020 & 0.046 & 0.036 & 0.057 & 0.007 & 0.022 & 0.023 & 0.053 & \textbf{0.014} & 0.082 \\
    \hline
    \multirow{2}{4em}{RSNet} &BHD & 0.263 & 0.282 & 0.343 & 0.265 & 0.122 & \textbf{0.117} & 0.208 & 0.312 & 0.242 & 0.307 \\
    &CD & 0.030 & 0.040 & 0.040 & 0.032 & 0.009 & \textbf{0.011} & 0.035 & 0.044 & 0.037 & 0.057 \\
    \hline     
    \end{tabular}
\end{adjustbox}
    \label{tab:kp_corres}
    \vspace{-3mm}
\end{table*}

==> tables/label_sdf_accuracy.tex <==
\begin{table*}[t]%[htb]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    & Mean & Airplane & Bath & Chair & Car & Guitar & Knife & Laptop & Motor & Table & Vessel \\
    \hline
    Top-1 &76.82 & 76.78 & 58.17 & 93.44 & 80.87 & 86.09 & 67.5 & 100.0 & 57.16 & 99.18 & 49.07 \\
    Top-3 &91.58 & 92.47 & 82.32 & 98.4 & 96.1 & 98.06 & 91.67 & 100.0 & 79.66 & 99.62 & 77.52 \\
    Top-5 &94.8 & 96.02 & 86.43 & 98.94 & 98.74 & 98.72 & 98.75 & 100.0 & 87.47 & 99.66 & 83.23 \\
    \hline
    \end{tabular}
    \caption{Top-1,3,5 accuracy for semantic label prediction}
    \label{tab:label_acc}
    \vspace{-2mm}
\end{table*}

==> tables/semantic_comp.tex <==
\begin{table}[t]%[htb]
    \caption{Comparison results of semantic label prediction with top-1, top-3, and top-5 accuracy (percentage). The vanilla method directly classifies our predicted keypoints using MLP.}
    \centering
    \begin{tabular}{l|c|c|c}
    \hline
         Method & Top-1 & Top-3 & Top-5 \\
         \hline
         Vanilla & 10.89 & 28.43 & 43.69 \\
         \hline
         Ours & \textbf{76.82} & \textbf{91.58} & \textbf{94.80} \\
    \hline
    \end{tabular}
    \label{tab:label_comp}
    \vspace{-2mm}
\end{table}
